FlowFusion: Dynamic Dense RGB-D SLAM Based on Optical Flow

Dynamic environments are challenging for visual SLAM since the moving objects occlude the static environment features and lead to wrong camera motion estimation. In this paper, we present a novel dense RGB-D SLAM solution that simultaneously accomplishes the dynamic/static segmentation and camera ego-motion estimation as well as the static background reconstructions. Our novelty is using optical flow residuals to highlight the dynamic semantics in the RGB-D point clouds and provide more accurate and efficient dynamic/static segmentation for camera tracking and background reconstruction. The dense reconstruction results on public datasets and real dynamic scenes indicate that the proposed approach achieved accurate and efficient performances in both dynamic and static environments compared to state-of-the-art approaches.

==> ral-reviews.tex <==
ReportOn19-1786v1.txt
Based on the reviews and my own evaluation, this work is overall solid
and has some technical merits. However, there are a few major concerns,
including insufficient comparative experiments and non-competitive
performance of the results with existing approaches (including the
authors' previous work). The authors are also suggested to provide a
clear statement of the novelty and contribution of this work compared
to other similar studies. Finally, the reviewers complained about the
presentation of the paper. The authors are suggested to improve the
work by these feedback comments. 

Review75647(Reviewer3)Of19-1786v1.txt

This paper presents a dense RGB-D SLAM algorithm that reconstruct the
static background together with dynamic/static segmentation and camera
ego-motion estimation in dynamic environments. Publicly available
datasets are used to validate the proposed algorithm and compared to
three of the state-of-art dynamic RGB-D SLAM algorithms.

The paper is overall well organised. The main contribution is using
optical flow residuals to highlight the dynamic semantics in the RGBD
point clouds and provide efficient dynamic/static segmentation. This
idea is interesting and works well in the experiments and comparison.

Some comments and suggestions to the authors:

In Section III.A Eq (1), when estimating the camera motion, a joint
optimisation of both photometric and geometric errors are minimised. As
the weights of nonlinear optimisation problem are always the inverse of
the covariance matrices of the measurements, the reviewer would like to
know how the two weights on the two terms are chosen and how they will
affect the results.
Eq (5), it is claimed “here we won’t provide a unique function of \pi
since it differs from different sensors types (such as pinhole camera,
stereo camera, and laser scanners).” While, as the paper is in the case
of RGB-D camera, I suppose it is the pinhole projection model and
please make Eq (5) as this specific case.

Section III.D, a metric is computed to combine three residuals. The
authors need to explain a bit in details how this metric is the ideal,
since normally combining different metrics together is always not
straight forward and cannot guarantee it is  better.

It will be good if the proposed algorithm can reconstruct both the
static background and the dynamic objects together simultaneously.

The experimental results are the strongest part of the paper, it uses
publicly available and real experimental datasets, compared with three
different state-of-art dynamic RGB-D SLAM algorithms. And showing the
proposed algorithm can work well in the static case is another
validation of the segmentation.


In the supplementary video, it is not necessary to show the results of
the four algorithms running together first, then show the same results
one by one separately. And some of the titles cannot be shown
completely in the video.

The presentation of the paper needs to be improved a lot. Below are
some comments w.r.t. this:

At the end of Page 2, “initial rigid motion guess” should be “initial
guess of the rigid motion”.

Page 3, below Eq (3), “which is …, which is…”.

Page 3, below Eq (5), “the projecting of a from a world coordinate
point to the camera plane”.

Page 3, below Eq (6), “high non-linear” should be highly nonlinear.

Page 4, below Eq (10), “we computer its dynamic level” should be
compute.

Page 4, the last paragraph, E(b) should be E_G(b).

In video, what does “hard dynamic” mean?

i
Review79353(Reviewer9)Of19-1786v1.txt

===================================
Summary
===================================
The paper introduces optical flow residuals to the energy function to
highlight the dynamic semantics in the RGB-D point clouds and assist
background reconstruction. Experiments on publicly available dataset
demonstrate that the proposed method is effective.
===================================
Comments
===================================
The main contribution of this paper is using optical flow residual in
camera tracking and background reconstructions. But the author doesn't
provide comparative experiments with and without that residual. 

The experiments are insufficient. The TUM RGB-D Dataset has 9 sequences
in the category of dynamic objects. The author's previous work
PoseFusion(PF) contains test results on 6 sequences. But this paper
only shows experiments on 2 sequences (fr3/walk_xyz and
fr3/walking_static). I wonder whether the FlowFusion(FF) works on ohter
sequences.

The results are not competitive enough. Compared with the author's
previous work PoseFusion(PF), although the FF outperforms the PF on
certain sequences, the PF has lower translation error and rotation
error on average.

The author said that the proposed optical flow residuals based
static/dynamic semantic segmentation method achieved efficient dynamic
foreground PCDs extraction performances in RGB-D benchmarks and Fig.6
shows the FlowFusion(FF) experimental result. But there is no
comparison with other methods to support the idea.
===================================
Spelling / Typos / Format
===================================
The paper seems to use the wrong template. The font size of the legend
should not be the same as the body. 

In equation (13), \delta_{t} and \delta_{b} should be \theta_{t} and
\theta_{b} as explained between equation (11) and equation (12).

\sout{Some references are inconsistent. [5] and [7] are both from
International Conference on Robotics and Automation (ICRA), one of
which wrote the full name and the short name while the other only wrote
the short name.
}

Review82005(Reviewer17)Of19-1786v1.txt

The paper introduces a SLAM algorithm that accounts for moving objects
in the environment. The authors introduce an algorithm that factors out
moving objects using optical flow, and the reconstruction result is on
par with the state-of-the-art approaches.

The overall writing of the paper is good and I appreciate authors for
providing clear diagrams of network structures and algorithms. The
formulations of the approach make sense and the descriptions are clear
as well. Experimental results demonstrate that the system can achieve
reasonable results.

I have a few questions regarding the paper:
- The computational speed of the system is not reported, given that
there are multiple steps in the system that require slightly more
complicated energy minimization steps
- The experimental results seems to make sense, but the performance is
not the state-of-the-art. It'll be good if authors can provide more
discussions about why the proposed system may potentially achieve
slightly worse results. It'll be better if authors can provide
comparisons in videos or visualizations.
- The citations are adequate, but there are already several published
works on SLAM systems that account for moving landmarks, such as
"Robust Graph SLAM in Dynamic Environments with Moving Landmarks, by
Lingzhu Xiang, Zhile Ren, Mengrui Ni, Odest Chadwicke Jenkins, IROS
2015". There are also several works that use semantic segmentations to
factor out moving objects and backgrounds in scene flow, such as
"Bounding boxes, segmentations and object coordinates: How important is
recognition for 3D scene flow estimation in autonomous driving
scenarios? By A. Behl, O. H. Jafari, S. K. Mustikovela, H. A. Alhaija,
C. Rother, and A. Geiger, ICCV 2017 " and "Cascaded Scene Flow
Prediction using Semantic Segmentation, by Zhile Ren, Deqing Sun, Jan
Kautz, Erik Sudderth, 3DV 2017"
